Fault-tolerant linear solvers via selective reliability

Energy increasingly constrains modern computer hardware, yet protecting computations and data against errors costs energy. This holds at all scales, but especially for the largest parallel computers being built and planned today. As processor counts continue to grow, the cost of ensuring reliability consistently throughout an application will become unbearable. However, many algorithms only need reliability for certain data and phases of computation. This suggests an algorithm and system codesign approach. We show that if the system lets applications apply reliability selectively, we can develop algorithms that compute the right answer despite faults. These "fault-tolerant" iterative methods either converge eventually, at a rate that degrades gracefully with increased fault rate, or return a clear failure indication in the rare case that they cannot converge. Furthermore, they store most of their data unreliably, and spend most of their time in unreliable mode. We demonstrate this for the specific case of detected but uncorrectable memory faults, which we argue are representative of all kinds of faults. We developed a cross-layer application / operating system framework that intercepts and reports uncorrectable memory faults to the application, rather than killing the application, as current operating systems do. The application in turn can mark memory allocations as subject to such faults. Using this framework, we wrote a fault-tolerant iterative linear solver using components from the Trilinos solvers library. Our solver exploits hybrid parallelism (MPI and threads). It performs just as well as other solvers if no faults occur, and converges where other solvers do not in the presence of faults. We show convergence results for representative test problems. Near-term future work will include performance tests.

==> future.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Future work}\label{S:future}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
%% FIXME (mfh 27 Sep 2011) Flexible CG might require storing the whole
%% search space, just like GMRES.  I need to check.  Is this also the
%% case for Flexible QMR?
%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Inner / outer iteration balance}\label{S:future:balance}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Our work does not currently address the balance between the number of
inner and outer iterations.  Some linear systems need many Krylov
subspace iterations to converge, while others only need a few.  Users
may not know the number of required iterations in advance.  FT-GMRES
currently conservatively stops inner solves after a fixed iteration
count.  A smarter strategy could mix more reliable fault detection and
convergence metrics to pick the inner solves' stopping criteria
adaptively.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Cheaper outer iterations}\label{S:future:outer-iter}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Our inner-outer iteration framework accommodates many different
combinations of solvers.  It only requires that the outer iteration be
``flexible,'' that is, that the preconditioner may change between
iterations.  We chose Flexible GMRES as the outer iteration because of
its promise of eventual convergence.  However, this guarantee comes at
a price: the number of basis vectors it must store grows linearly with
the number of (outer) iterations.  Depending on the required number of
outer iterations and the cost of storing those vectors reliably (as
the outer solver must do), it may be attractive to use an algorithm
which stores only a constant number of vectors.

One limitation is that corrupted matrix or preconditioner applications
in the inner iteration may cause the inner solve to appear as a
``nonsymmetric preconditioner,'' from the perspective of the outer
iteration.  Even if the uncorrupted matrix $A$ is symmetric,
nonsymmetric inner solves will make the outer iteration's
preconditioned operator nonsymmetric.  Thus, it is important to use an
outer iteration that does not assume symmetry.  Flexible QMR
\cite{szyld2001fqmr} is a nonsymmetric method that uses a constant
number of vectors.

\begin{comment}
  its proimse that it either eventually converges, or that it quickly
  detects stagnation of the outer iteration due to unlucky inner
  solves.

All inner-outer Krylov iterations without data or arithmetic
corruption converge eventually \cite{simonici2003flexible} -- not
quite... It's more like either the subspace keeps growing, or the
iteration stagnates...
\end{comment}

%%
%% QUESTION: Does Flexible QMR also promise eventual convergence, when
%% used as an inner-outer iteration?  NO -- it doesn't because it
%% doesn't keep the outer basis, so unlucky inner solves may result in
%% stagnation, which can't be detected as easily... is that true?
%%

% There are flexible versions of other iterative methods besides GMRES,
% such as CG \cite{golub1999inexact} and QMR 


% Check the following references for Flexible CG:
% http://onlinelibrary.wiley.com/doi/10.1002/nla.1680010108/abstract


\begin{comment}
A number of algorithmic questions remain.

Number of iterations to spend in the inner iteration?
Do we restart the inner iteration?
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Software-enabled reliable memory}\label{S:future:storage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

One limitation of our reliable memory scheme is that it assumes only
fail-stop reliability.  Its reliability comes from its small memory
footprint, relative to the total memory used by the solver.  If a
memory region not marked unreliable experiences an uncorrectible ECC
fault, the operating system terminates the application.  This is
appropriate for some data, such as application code, loop counters, or
other control state.  There is no safe way to recover when such data
are corrupted other than to restart globally from a checkpoint, since
the program may be in an arbitrary invalid state and there is no way
for the application to introspect this state.

However, much of FT-GMRES' data, such as the matrix $A$, the
preconditioner(s), and the right-hand side $b$, could be stored
reliably using a software error-correcting code.  This would require a
more sophisticated fault response framework, so that memory faults
detected in reliable memory could initiate a still local but more
complex correction process.  There are many promising encoding schemes
that work well with floating-point data.  All of them trade additional
storage and computation for reliability, so it would be necessary to
analyze the costs of this approach.  It may or may not save energy or
improve performance over a fail-stop approach to reliable data.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Algorithmic fault detection}\label{S:future:alg-fault}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Krylov methods have a number of invariants.  Violation of these
invariants could indicate corrupted data or arithmetic operations, as
Chen et al.\ \cite{???} point out.  

Using easily-checked invariants of the inner Krylov method in order to
detect faults

This approach would be more likely to detect transient faults than
persistent ones.  For example, if the matrix $A$ was corrupted into a
nonsingular matrix $\tilde{A}$ before a GMRES inner solve cycle, and
that corruption persisted through the whole inner solve, none of
GMRES' invariants would be violated.


